ANALOGYKB: Unlocking Analogical Reasoning of Language Models with A Million-scale Knowledge Base

Analogical reasoning is a fundamental cognitive ability of humans. However, current language models (LMs) still struggle to achieve human-like performance in analogical reasoning tasks due to a lack of resources for model training. In this work, we address this gap by proposing ANALOGYKB, a million-scale analogy knowledge base (KB) derived from existing knowledge graphs (KGs). ANALOGYKB identifies two types of analogies from the KGs: 1) analogies of the same relations, which can be directly extracted from the KGs, and 2) analogies of analogous relations, which are identified with a selection and filtering pipeline enabled by large language models (LLMs), followed by minor human efforts for data quality control. Evaluations on a series of datasets of two analogical reasoning tasks (analogy recognition and generation) demonstrate that ANALOGYKB successfully enables both smaller LMs and LLMs to gain better analogical reasoning capabilities.

==> tables/060ablation.tex <==
\setlength\tabcolsep{2pt}
\begin{table}[t]
  \centering
  \small
    \begin{tabular}{lccccccc}
     \toprule
    \textbf{Method} & \textbf{E-KAR}  & \textbf{BATS}  & \textbf{U2}    & \textbf{U4}    & \textbf{Google} & \textbf{SAT}   & \textbf{Mean} \\
    \midrule
    FT    & 46.70  & 78.20  & 46.05  & 40.04  & 96.90  & 51.60  & 59.92 \\
    \cdashlinelr{1-8}
    PT$_{R}$ & 29.77 & 28.84 & 21.49 & 25.92  & 19.20  & 15.73 & 23.49 \\
    \ \ + FT & 35.62 & 38.30   & 24.12 & 30.09 & 32.60  & 24.03 & 30.79 \\
    PT$_{E}$ & 42.74 & 80.60  & 43.42 & 43.28& 94.20 & 49.25 & 58.92 \\
    \ \ + FT & 51.90 & 90.55  & 71.49 & 63.88 & {97.80} & 57.86 & 72.25 \\
    PT & 46.18  & 79.54    & 50.00  & 46.99 & 96.20  & 49.26 & 61.36 \\
    \ \ + FT & \textbf{53.43 } & \textbf{90.93 } & \textbf{87.28 } & \textbf{76.15 } & \textbf{97.80 } & \textbf{59.05 } & \textbf{77.44 } \\
    \bottomrule
    \end{tabular}%
    \caption{An analogy recognition task results in ablation. 
    [\todo: turn it into histograms, @ysy]}
  \label{tab:ablation}%
\end{table}%
    
    

==> tables/090meta.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[t]
  \centering
  \small
   \begin{tabular}{lcl}
    \toprule
    \textbf{Type} & \textbf{Num.} & \multicolumn{1}{c}{\textbf{Example}} \\
    \midrule
    Meta Relation & 35    & \makecell[l]{Meta: head of organization\\Relation: chief executive officer, \\head of state, director, etc.} \\
    \bottomrule
    \end{tabular}%
    \caption{The meta relations and entity schemas to explain the similar-relational analogies.}
  \label{tab:meta}%
\end{table}%


==> tables/130GPT-3_prompt_for_EKAR.tex <==
\begin{table}[t]
\footnotesize
  \centering
    \begin{tabularx}{\linewidth}{X}
    \toprule
    %\rowcolor[gray]{0.95}\multicolumn{1}{c}{\textbf{Analogy Recognition Task}}
    %\midrule
    \makecell[l]{
    \color{gray}{/* \textit{Task prompt} */}\\
    Find the most analogous candidate answer that follows the \\ relations in the query.\\
    \\
    \color{gray}{/* \textit{Examples} */} \\
    Question: candy:sugar\\ Choice:\\ A: wig:hair\\ B: ocean:atmosphere\\ C: cry:scream\\ D: house:roof\\ Please choose A, B, C or D.\\ Answer: A \\
    \\
    \color{gray}{/* \textit{Examples w COT} */} \\
    Question: candy:sugar\\ Choice:\\ A: wig:hair\\ B: ocean:atmosphere\\ C: cry:scream\\ D: house:roof\\ Please choose A, B, C or D.\\ Answer: Candy is made of sugar and wig is made of hair. \\Ocean is made of water. Cry is not made of scream. \\ House is not made of roof. So the answer is A \\
    ...\\
    \\
    \color{gray}{/* \textit{Test data} */} \\
    Question: raphael:painter\\ Choice:\\ A: andersen:plato\\ B: reading:berkshire\\ C: marx:philosopher\\ D: tolstoi:edison\\ Please choose A, B, C or D.\\ Answer: \color[rgb]{0,0.39,0}C} \\
    \bottomrule
    \end{tabularx}
  \caption{Examples of prompt for LLMs for analogy recognition task. Generated texts by LLMs are {\color[rgb]{0,0.39,0}\textit{highlighted}}.
  }
  \label{tab:GPT-3_prompt_for_EKAR}
\end{table}


==> tables/150InstructGPT.tex <==
%\setlength\tabcolsep{2pt}
\begin{table*}[t]
  \centering
  \small
    \begin{tabular}{lccccccc}
     \toprule
    \textbf{Method} & \textbf{E-KAR}  & \textbf{BATS}  & \textbf{U2}    & \textbf{U4}    & \textbf{Google} & \textbf{SAT}   & \textbf{AVG.} \\
    \midrule
    InstructGPT$_{0}$ & 32.44  & 57.78  & 47.80  & 46.99   & 78.40  & 37.39 & 50.13  \\
    InstructGPT$_{1}$ & 38.93  & {81.90}  & 50.00  & {52.78} & 91.60  & 48.96 & {60.70}\\
    InstructGPT$_{2}$ & 40.46 & 78.89    & {53.94} & 50.00  & {93.00} & 44.21 & 60.08  \\
    InstructGPT$_{3}$ & 38.93  & 75.37    & 48.24  & 45.37 & 91.40  & 43.02 & 57.06  \\
    \cdashlinelr{1-8}
    InstructGPT$_{0}$ w/ & 41.21  & 70.34  & 53.94  & 52.78  & 83.00  & 45.99  & 57.88  \\
    InstructGPT$_{1}$ w/ & 44.27  & 71.34  & 60.08  & 57.86  & 84.80  & 47.48  & 60.97  \\
    InstructGPT$_{2}$ w/ &46.18  & 75.36  & 56.57  & 55.55  & 87.60  & 46.88  & 61.36  \\
    InstructGPT$_{3}$ w/ &46.94  & 71.35  & 57.89  & 55.32  & 84.20  & 45.69  & 60.23  \\
    \bottomrule
    \end{tabular}%
    \caption{Accuracy results of InstructGPT 175B on the analogy recognition task.}
  \label{tab:InstructGPT_evaluation}%
\end{table*}%

==> tables/170comet.tex <==
%\setlength\tabcolsep{1.8pt}
\begin{table*}[t]
  \centering
  \small
    \begin{tabular}{lccccccc}
     \toprule
    \textbf{Model} & \textbf{E-KAR} & \textbf{BATS}  & \textbf{U2} & \textbf{U4} & \textbf{Google} & \textbf{SAT} & \textbf{Mean} \\
    \midrule
    GPT-2-XL & 29.01 & 25.73  & 23.68 & 28.01 & 33.20  & 25.82 & 27.58 \\
    BART-L  & 29.77 & 31.18  & 25.44 & 32.18 & 41.80  & 25.52 & 30.98 \\
    COMET$_{G}$ & 28.62 & 30.29  & 30.26 & 31.94 & 36.80  & 29.08 & 31.17 \\
    COMET$_{B}$ & 36.64 & 37.97   & 33.33 & 40.50 & 47.60  & 35.60 & 38.61 \\
    \method$_{G}$ & 40.18 & 48.95 & 35.59 & 41.32  & 53.86 & 37.62	& 42.92  \\
    \method$_{B}$ & \textbf{42.06} & \textbf{51.36}  & \textbf{40.70}  & \textbf{42.57} & \textbf{59.40}  & \textbf{41.45} & \textbf{46.26} \\
    \bottomrule
    \end{tabular}%
    \caption{Compare the word embedding trained upon \method and commonsense reasoning data.}
  \label{tab:comet}%
\end{table*}%

